Falling Trees: A Model Class for Interpretable Risk Prioritization

Many real-world decisions require prioritizing high-risk cases, such as clinicians prioritizing high-risk patients before lower-risk ones. Falling rule lists (FRLs), which are ordered if--then rules with monotonically decreasing risks, provide an interpretable framework for such tasks; however, their single-path structure yields a highly restricted model class. We introduce falling trees, a new family of interpretable models that enforces the same monotonic risk constraint while permitting tree-structured branching. We present GRAVITree, a novel dynamic-programming-with-bounds algorithm for learning the Rashomon set of falling trees under depth and branching constraints. Our formulation can interpolate between rule lists and full decision trees, enabling user-desired model expressivity. In a new clinical dataset and in many public classification benchmarks, falling trees match or outperform FRLs and other interpretable baselines, often producing more sparse decisions for high-risk instances. Our results show that falling trees strike a practical balance between interpretability, expressiveness, and risk prioritization for high-stakes settings.

==> sections/theoretical_analysis.tex <==
We now describe some theoretical properties that make \gravitree particularly compelling, not only in the trees it outputs, but also how it leverages falling constraint based pruning.
Because the hypothesis class of FRLs is a subset of that of falling trees, the best falling tree will have training error no less than the best FRL. In some cases, as discussed below, falling trees can also achieve arbitrarily low error while FRLs can be arbitarily bad. 







% Alongside being more expressive model class than FRLs, falling trees also pose a major advantage compared to regular trees. A falling tree will exhibit lower decision sparsity on the class of interest compared to a regular tree with the same error rate. 

% \begin{proposition}[Falling trees induce higher positive-class sparsity]
% \label{prop:sparsity}
% Let $T_1$ and $T_2$ be two decision trees trained on the same sample $D$, and suppose they achieve the same empirical misclassification loss on $D$. Let $\mathrm{sp}^+(T)$ denote the decision sparsity of the positive class:
% \[
% \mathrm{sp}^+(T) \;:=\; \mathbb{E}_{\bx,y \in D}\!\left[\, \mathrm{depth}(T(\bx)) \;\middle|\; y=1 \right].
% \]
% If $T_2$ is falling and $T_1$ is not, then
% \[
% \mathrm{sp}^+(T_2) \;\le\; \mathrm{sp}^+(T_1).
% \]
% i.e., falling trees have greater decision sparsity for the positive class.
% \end{proposition}

